SiEVE: Semantically Encoded Video Analytics on Edge and Cloud

Recent advances in computer vision and neural networks have made it possible for more surveillance videos to be automatically searched and analyzed by algorithms rather than humans. This happened in parallel with advances in edge computing where videos are analyzed over hierarchical clusters that contain edge devices, close to the video source. However, the current video analysis pipeline has several disadvantages when dealing with such advances. For example, video encoders have been designed for a long time to please human viewers and be agnostic of the downstream analysis task (e.g., object detection). Moreover, most of the video analytics systems leverage 2-tier architecture where the encoded video is sent to either a remote cloud or a private edge server but does not efficiently leverage both of them. In response to these advances, we present SIEVE, a 3-tier video analytics system to reduce the latency and increase the throughput of analytics over video streams. In SIEVE, we present a novel technique to detect objects in compressed video streams. We refer to this technique as semantic video encoding because it allows video encoders to be aware of the semantics of the downstream task (e.g., object detection). Our results show that by leveraging semantic video encoding, we achieve close to 100% object detection accuracy with decompressing only 3.5% of the video frames which results in more than 100x speedup compared to classical approaches that decompress every video frame.

==> background.tex <==
\section{Background}\label{sec:background}
%\subsection{Neural Networks}

%{\bf Neural Network (NN) Architecture}: A neural network consists of a series of connected layers that can process a high-dimensional input image and output a simpler representation. Each layer of a convolutional NN corresponds to a step in computation: these layers include convolutional layers (that combine nearby pixels via convolution operators), pooling layers (that reduce the dimensionality of the subsequent layers), rectified linear unit (ReLU) layers (that perform a non-linear transformation), fully connected layers (that perform matrix additions, multiplications), and a softmax layer (that outputs the final prediction based on the previous layers. 


%As illustrated below [1], combining multiple such layers in a “deep” architecture and by fitting the appropriate weights of the computation (i.e., the “neurons”) between stages, NNs can learn the structure of common objects and detect their presence
%and absence in a given image. Depending on the task, the best model architecture (e.g., configuration
%of layers) varies, but the overwhelming trend has been to build
%deeper models given more training data.


%{\bf NN Training}: Training NNs consists of fitting appropriate weights to a given architecture such that the overall empirical error on a given set of labeled training data is minimized. This process is computationally expensive, but is now supported by a wide range of software frameworks such as Google TensorFlow, Torch and Caffe. To train an object detector on video, we would first label a portion of a video (or set of videos) by hand, marking which frames contained cars and which did not. Subsequently, we would feed each frame to a NN training framework. Due to the computational cost of training NNs, companies and researchers have also published hundreds of pre-trained models, each representing thousands of hours of CPU and GPU training time. 
%{\bf NN Inference:} Applying NNs to video consists of passing individual video frames to a NN, one frame at a time. That is, to detect objects in video, we evaluate the NN repeatedly, once per frame. In our system, we focus on optimizing the speed of NN inference. 

%For example, we decide which video frames to feed to a pre-trained object detection/classification model and we decide which part of the NN inference is executed on the private/local compute resources (i.e., edge) and which part is executed in the remote compute resources (i.e., cloud) 


{\bf Video Encoders:} A video consists of a sequence of frames that have spatial similarity. Video encoder is the piece of software or electric circuit that makes use of such spatial similarity to {\it compress} a video. To compress a video, state-of-the-art video encoders (e.g., h.264, h.265) choose only a subset of the video frames (known as I-frames or key-frames) to be encoded in the full resolution. The rest of the frames are known as Predicted frames (P-frames), and Bidirectional frames (B-frames) and they only encode the difference between them and one or more I-frames. 
 A video can thus be seen as a sequence of clips where each clip is known as a group of pictures (GOP). Each GOP starts with one I-frame and is followed by an arbitrary number of P-frames and B-frames. %as shown in Figure~\ref{fig:encoded_video}.
 Video encoders have two configurable parameters that control the number of I-frames and the duration between two I-frames. The parameters are:
 
% \begin{figure}[t]
%  	\centering
%  	\includegraphics[width=\linewidth]{figures/encoded_video.png}
%	\caption{Example of a compressed video.}
	%\label{fig:encoded_video}
%\end{figure}
 
 \begin{enumerate}
 \item {\bf scenecut threshold:} a threshold on the motion difference between two consecutive frames. If motion is less than scenecut threshold, a new I-frame is created.
  \item {\bf GOP size:} the duration between two I-frames (key frames). It is essentially the number of P and B frames between two I-frames.
  
  %It has a default value of 250 frames which means that if the difference between consecutive frames is small and the {\it scenecut threshold} does not decide to create a new I-frame, then after 250 frames, the video encoder will automatically create a new I-frame regardless of the difference between the current frame and the previous frame.
  
  
  %\item {\bf Scenecut threshold}: This parameter determines if a given frame is encoded as an I-frame or a P-frame. To do this, video encoder keeps track of the difference (i.e., motion) between every frame and the previous frame in the video. If the difference is below the scenecut threshold, a new GOP is created and its initial I-frame is the given frame. Otherwise, the given frame is encoded as a P-frame or B-frame in the previous GOP. 
    %\item {\bf GOP size:} This parameter controls the maximum number of frames in a GOP (i.e., the maximum number between two I-frames). It has a default value of 250 frames which means that if the difference between consecutive frames is small and the {\it scenecut threshold} does not decide to create a new I-frame, then after 250 frames, the video encoder will automatically create a new I-frame regardless of the difference between the current frame and the previous frame. Hence, the GOP size is hard limit for the number of P or B frames between two I-frames.
     \end{enumerate}
     %If the GOP size is set to a large a value, each P-frame will depend on an I-frame that is more than 250 frames away which could affect the decoding speed and the quality of the decoded frame.  
     
     %It has a default video of 250 frames per GOP to balance the tradeoff between high compression ratio and fast decoding. If the GOP size set to be too large, the video will have less I-frames, and it is more compressed. However, while the video is being decoded, each P-frame will depend on the I-frame that is more than 250 frames away which could affect the decoding speed and the quality of the decoded frame. 

{\bf Video Decoders:} Video decoder is the piece of software or electric circuit that does the oppposite operation to video encoders. Video decoders convert a compressed video back to a sequence of frames. In the process of video decoding, each type of frames (i.e., I, P or B) is treated differently. In our discussion, we focus on I and P-frames only because they are available in both live and pre-recorded videos, however, B-frames exist only in pre-recorded videos and they can be converted to P-frames. The I-frames are the simplest to decode because they carry all the pixel information and they are {\it independent} of other frames. Decoding an I-frame is the same as decoding a still image such as a JPEG images. On the other hand, P-frames only encode the motion between the current frame and the previous frame. Hence, decoding a P-frame requires decoding all the previous P-frames all the way back to the closest I-frame which means that decoding P-frame is significantly more expensive than decoding I-frames.


%if the current frame is P-frame and the previous is an I-frame, then the previous I-frame is used with the motion information in the current P-frame to decode the current P-frame. However, if the current frame is a P-frame and the previous frame is also a P-frame then all the previous P-frames up to the closest I-frame have to be decoded first.

%{\bf Summary:} With reference to the object detection workflow shown in Figure~\ref{fig:obj_det}, we conclude that we can significantly speed up video object detection by extracting and decoding I-frames rather than decoding the entire video with both I and P-frames. We present a system design the focuses on analyzing I-frames only in Section~\ref{sec:system}. However, by focusing on I-frames only, we are missing a big portion of the video that might contain important events. Therefore, one of the main contributions of this paper is to tune video encoder parameters (i.e., GOP size and scenecut threshold) to produce I-frames when a {\it semantic} event happens such as a car entering or leaving the scene. We provide more details about our semantic video encoder in Section~\ref{sec:encoder}. Moreover, we propose a neural network partitioning technique to speed up the object detection on the extracted I-frames. The details of NN partitioning is presented in Section~\ref{sec:nn}.


%Extracting I-frames only esssentially means that all P-frames can be dropped and I-frames can be treated as still images. This makes video decoding significantly faster because the decoding happens through seeking I-frames in a {\it compressed video} rather than decoding every frame. 

%by focusing on decoding each frame of the video  We conclude that  only is significantly faster than . 

%P-frames and B-frames are only concerned about %capturing the motion
%and every pixel information  but it’s a complete image in the sense that every pixel is there.

% In our system, we focus on analyzing I-frames only because they can be decoded independently unlike P and B-frames which are encoded with reference to a previous I-frame. This makes video analysis significantly faster and with significantly less bandwidth consumption because the analysis happens through seeking I-frames in a {\it compressed video} rather than decoding every frame. 
 
 %However, by focusing only in I-frames, we are missing a big portion of the video that might contain important events. Therefore, one of the main contributions of this paper is to tune video encoder parameters (i.e., GOP size and scenecut threshold) to produce I-frames when a {\it semantic} event happens such as a car entering or leaving the scene. We provide more details about our semantic video encoder in Section~\ref{sec:encoder}.
 
 %controls how many I-frames appear in a video. I-frames 
 %The video encoder decides whether a given frame should encoded as an I-frame, P-frame or B-frame based on a parameter called {\it scenecut threshold} (i.e., sc threshold).  
 



%This is for several
%reasons. First, NNs are almost always trained on static images, not on moving video. Therefore, evaluating them on video by converting them to a series of static images is easy (if expensive). Second,
%historically, the resurgence of interest in NNs has been driven by
%competitions such as ImageNet, in which the only metric of interest  is accuracy, not inference speed. The difference between the firstand
%second-place in ImageNet 2016’s object recognition competition
%was 0.72\% (2.99\% vs. 3.71\% top-5 classification error; in contrast,
%humans achieve approximately 5.1\% error). Therefore, with few
%exceptions [37], accelerated methods are not favored by the most prestigious competitions in the field. Finally, the handful of object recognition CNNs that are optimized for inference time primarily
%use “real time” (i.e., 30 fps) as a target [79–81], aiming to evaluate
%one video in real time on a GPU. In contrast, we are interested in
%scaling to thousands of hours of video, possibly from thousands of
%data feeds, for the purposes of large-scale video classification; real time performance is not nearly fast enough for our target scale.

==> nn.tex <==
\section{Neural Network Partitioning}\label{sec:nn}

The frames that undergo neural network inference are the I-frames produced by the semantic video encoder and extracted by the {\it I-frame seeker} shown in Figure~\ref{fig:overview}. The I-frames of the semantically encoded video are the ones more likely to have objects that are different than the previous frame. The I-frames are decompressed in the same way still JPEG images are decompressed and they are passed to the neural network to identify the actual objects that appear in each I-frame. 
The I-frames can come from several semantically encoded videos, each corresponding to a different camera. In this section, we describe a technique to partition a neural network across edge and cloud compute resources to minimize the execution time of a stream of I-frames. We start by describing the neural network model and the data model, and the intuition behind the approach. Then we formally define the problem and describe the algorithm to solve it.   
%Neural networks have long been treated as a blackbox model with systems like Clipper~\cite{} and Tensorflow Serving. The key idea in our approach is leveraging 

%Existing neural network inference systems, such as Clipper~\cite{}, TensorFlow Serving~\cite{}, Rafiki~\cite{} focus
%mainly on ease of deployment, where the entire neural network is considered as a black box and deployed into one Docker container. However, they miss the opportunity of leveraging hierarchical clusters through deploying some layers of the neural network on the edge server near the data source and the rest of the layers in a remote cloud. In the following we describe how we model the neural network and the data fed to it. Then we describe the key idea behind the approach and the detailed algorithms steps. 

%\begin{table}[t]\caption{Table of Notation}
%\begin{center}
%\begin{tabular}{r c p{6cm} }
%$m$ & $=$ & number of layers in a neural network\\
%$L_i$ & $=$ & Layer $i$ in a neural network\\
%$f_i$ & $=$ & Frame $i$ in a chunk of frames \\
%$n$ & $=$ & Total number of frames in a chunk \\

%$L_i@E$ & $=$ & Execution time of layer $i$ in the edge \\
%$L_i@C$ & $=$ &  Execution time of layer $i$ in the cloud  \\
%$L_i \rightarrow L_j@E$ & $=$ & Execution time of layer $i$ to layer $j$ in the edge \\
%$L_i \rightarrow L_j@C$ & $=$ & Execution time of layer $i$ to layer $j$ in the cloud \\
%$t_{chunk}\big(n, L_x\big)$ & $=$ & Completion time of a chunk of $n$ frames  when the NN is partitioned after layer $L_x$ \\
%$D_{L_i}$ & $=$ & Size (bytes) of output data/tensor of layer $L_i$ \\
%$B_{E,C}$ & $=$ & Bandwidth (bytes/sec) between edge and cloud \\
%$tr{(E\xrightarrow{\text{$D_{L_i}$}}C)}$ & $=$ & Transmission time (sec) between edge and cloud


%\bottomrule
%\end{tabular}
%\end{center}
%\label{tab:notation}
%\vspace{-0.3in}

%\end{table}

{\bf Neural Network Model:}
We model the neural network as a sequence of layers. Each layer is a processing operation such as convolution or matrix multiplication. A link from layer $L_1$ to layer $L_2$ means that for a given video frame $f_j$, $L_1$ has to be applied before $L_2$ and the output of $L_1$ is the input for $L_2$.

{\bf Data Model:}
We model the data as an unbounded stream of video frames $f_j$ that can come from one or more camera sources. The frames that undergo neural network inference are the I-frames produced by the semantic video encoder. We aggregate a sequence of video frames into {\it chunks} where each chunk has duration $T$. The $k^{th}$ chunk $chunk_k$ can be defined as $chunk_k= \langle f_{1}^{k}, f_{2}^{k}, \dots f_{n}^{k}\rangle$, where $n$ is the chunk size. The chunk duration/size is an application defined parameter to define how often the partitioning algorithm gets invoked to dynamically change the partitioning.

%In the rest of the paper we deal with a chunk of data. The chunk duration/size is an application defined parameter to define how often does the partitioning algorithm get invoked to dynamically change the partitioning.   

\begin{figure}[t]
  	\centering
  	\includegraphics[width=0.8\linewidth]{figures/example_4.pdf}
	\caption{Comparison between the execution time of a NN in three different cases: all layers on the edge (left), all layers on the cloud (middle), layers partitioned across edge and cloud (right) .}
	\label{fig:example}
	%\vspace{-0.1in}
\end{figure}


{\bf Approach Overview:} The key idea in our neural network partitioning approach is to allow processing a stream of video frames in a pipeline fashion. Pipelining allows utilizing both edge (E) and cloud (C) servers. For example, while the edge server is processing the first part of the neural network for the second video frame, the cloud server will be processing the second part of the neural network for the previous frame. Figure~\ref{fig:example} shows the execution and transmission time for executing a neural network in three different cases: (1) all layers of the NN are deployed on the edge server (left column), (2) all layers of the NN are deployed on the cloud server (middle column), and, (3) the NN is partitioned across edge and cloud (right column). Figure~\ref{fig:example} shows that the best completion time for one frame is the second case when all layers are on the cloud (300 ms). However, when we have a stream of 1000 frames, the best completion time is the third case (i.e., NN partitioning). The reason is \emph{pipelined execution} which means that when both edge and cloud are concurrently processing different frames, the completion time becomes bounded by the completion time of the edge partition only, which is the bottleneck layer in the example in Figure~\ref{fig:example}. Since the edge partition in this case accounts for one third of the entire execution time (160 ms/frame at the edge), the entire completion time is better than the other two cases (edge only and cloud only). 

{\bf Pipelined Execution:} To better illustrate how the completion time of a partitioned NN is calculated, we show an example of the pipelined execution in Figure~\ref{fig:pipeline}. Figure~\ref{fig:pipeline} depicts the execution for a {\it chunk} of three video frames. We denote the time to process layer 1 at the edge by $L_1 @ E$. Similarly, the times to process layer 2 to layer 3 at the cloud is denoted by $L_2 \rightarrow L_3 @ C$ and the transmission time of the intermediate data from the edge to the cloud is denoted by $tr_{E->C}$. From Figure~\ref{fig:pipeline}, we notice that at the same time that video frame 2 is being processed at the edge, video frame 1 is being transmitted over the network and processed at the cloud. The completion time of executing a chunk of $n$ frames on a neural network partitioned after layer $L_x$ is denoted by $t_{chunk}\big(n, L_x\big)$. For example, the completion time of the entire chunk of three frames partitioned after layer $L_1$ (shown 
in Figure~\ref{fig:pipeline}) is calculated as:

$\quad t_{chunk}\big(n=3, L_1\big) = 3*L_1@E + tr_{E->C} + L_2 \rightarrow L_3 @ C$

%$t_{chunk}\big(n=3\big, L_x)$, where $L_x$ is the  The completion time of the entire chunk of three frames  as shown in Figure~\ref{fig:pipeline} is calculated as:
%$t_{chunk}\big(3\big)=3*L_1@E + tr_{E->C} + L_2 \& L_3 @ C$$

\begin{figure}[t]
  	\centering
  	\includegraphics[width=0.9\linewidth]{figures/pipeline_3.pdf}
	\caption{Pipelined execution of 3 video frames ($n=3$) for the partitioned NN in the right column of Figure~\ref{fig:example}  .}
	\label{fig:pipeline}
		\vspace{-0.1in}

\end{figure}
We note that for a large chunk of frames $n$, the chunk completion time becomes bounded by the first term only, which is the one with the largest execution time in this example.
%$$t_{chunk}\big(n, L_1\big)=n* L_1@E + %tr_{E->C} + L_2 \rightarrow L_3 @ C %\simeq n*L_1@E $$
The general formula for chunk completion time for $m$ layers and $n$ video frames when partitioned after layer $L_x$ is:
\vspace{-0.1in}
\begin{equation}\label{eq:pipelining}
\begin{split}
t_{chunk}\big(n, L_x\big)=\underbrace{ \big(n - 1\big)* max\big( L_0\rightarrow L_x@E, tr_{E->C}, L_{x+1}\rightarrow L_{m} @ C \big)}_\textrm{queuing time}  \\  + \quad \underbrace{L_0\rightarrow L_x@E}_\textrm{exec. time on edge} +  \underbrace{tr_{E->C}}_\textrm{transmission time} +  \underbrace{L_{x+1}\rightarrow L_{m} @ C}_\textrm{exec. time on cloud}
\end{split}
\end{equation}

such that $L_0\rightarrow L_x@E$ denote the execution time of the first $x$ layers on the edge, and $L_{x+1}\rightarrow L_{m} @ C$ denotes the execution time of layer $x+1$ to layer $m$ on the cloud. The execution time of $x$ layers on the edge can be calculated as the sum of the execution times of its individual layers
%as follows: 
%\[ 
%L_0\rightarrow L_x@E= \left\{
%\begin{array}{ll}
%      \sum \limit_{i=1}^{i=x} L_i @ E & 0 < x \leq m \\
      
%       0 & x \leq 0 \\
%\end{array} 
%\right. 
%\]

%\[ 
%L_{x+1}\rightarrow L_m@C= \left\{
%\begin{array}{ll}
%      \sum \limit_{i=x+1}^{i=m} L_i @ C & 0 \leq x < m \\
      
%       0 & x \geq m \\
%\end{array} 
%\right. 
%\]

%The execution time of $x$ layers can be calculated as the sum of execution times of its individual layers. Similarly, The sum of the first $x$ layers on the edge can be calculated as the sum of each The two terms can be calculated as follows:



{\bf Problem definition:} Based on Equation~\ref{eq:pipelining}, we define the NN partitioning problem as finding the partitioning point $x$ that minimizes the chunk completion time $t_{chunk}\big(n, L_x\big)$. We formally define the problem as: $\quad x^* = \underset{x} {\mathrm{argmin}} \big(t_{chunk}\big(n,L_x\big)\big)$
 
%In this problem, we consider the chunk size $n$ an input parameter, however, we provide guidelines on how to choose the value of $n$ after we describe the algorithm steps.

%partitioning algorithm get invoked to dynamically change the partitioning
{\bf Algorithm Steps:} The following steps are performed offline once to find the best initial partitioning point and the system keeps monitoring online profiling information for the execution time of each NN layer and issues a re-partitioning when the profiling information deviates from the predicted execution times. %as we will describe later in this section.      
\begin{enumerate}
    \item {\bf Step 1 - Profile the execution and transmission times for each layer.}:  Each layer in the NN is associated with a {\it profile} which includes:
\begin{enumerate}
\item The cost of executing layer $L_i$ on a video frame $f_j$, when placed on each compute resource. Layer $L_i$ can be placed on an edge server $E$ or a cloud server $C$. Their corresponding execution times are $L_i @ E$ and $L_i @ C$.

%We assume that the data frames within chunk $ch_k$ have equal sizes therefore the execution cost is the same for all data frames.
% The execution cost is defined as $e_{o_i}=\{e_{i,E},e_{i,C}\}$. 

% The execution cost is measured by applying $o_i$ to $d_j$ on resource $r_l$ 
%It is defined as:
	 
 
 
%The execution time of operator $o_i$ when placed on of the $L$ resources.  $e_{i,l}(d_j))\stackrel{\text{def}}{=}$ A set of execution times of $o_i$ when applied to data frame $d_j$ on device $r_l$ 
\item The size of output data of layer $L_i$. We denote it as $D_{L_i}$ bytes.The output data of each layer is typically n-dimensional matrix (i.e., tensor) and its size can be derived from the resolution of the input frame. 

\item The transmission time of $L_i$ from the edge to the cloud, $tr(E\xrightarrow{\text{$D_{L_i}$}}C) = \frac{D_{L_{i}}}{B_{E,C}}$, where $B_{E,C}$ is the bandwidth (bytes/sec) from the edge to the cloud. 

%Since we assume that the data frames within a chunk have equal sizes, the output data of $o_i$ is the same for all data frames i.e. $\forall d_j^k \in ch_k\ D_{o_i}=D_{o_i}(d_j^k)$.
\end{enumerate}
    \item {\bf Step 2 - Evaluate the execution time at each possible partitioning point}: For a NN with $m$ layers, there are $m+1$ possible points to partition the NN including partitoning after layer 0 (i.e., everything is executed in the cloud) and partitioning after layer $m$ (i.e., everything is executed in the edge). We denote the layer that we partition after as $L_x$. For $x = \{0 \dots m\}$, we compute the execution time according to Equation~\ref{eq:pipelining}.
    
    \item {\bf Step 3 - Choose partitioning point}: From step 2, we get a set $S$ that contains the execution times at each partitioning point: 
    $S = \{t_{chunk}\big(n,L_x\big) \}_{x=0}^{x=m}$
    
    %$exec = %\{t_{chunk}\big(n,1\big),t_{chunk}\big(n,2\big), \dots ,t_{chunk}\big(n,m-1\big)\}$. 
    
    We choose the optimal partitioning point $x^*$ that yields the minimum execution time: $\quad x^*= \underset{x} {\mathrm{argmin}}\big(S \big)$
	%$$X^*=argmin(t_{chunk}\big(n,x\big)$$
\end{enumerate}

%{\bf Dynamic Repartitioning:}
%The profiling information collected in {\bf Step 1} is continuously monitored and logged by both the edge and cloud compute engines. After $k$ chunks, the edge compute engine reports the profiling information to the cloud controller. The cloud controller asks the NN partitioning service to compute a new partitioning point. If the new partitioning is different than the current partitioning point, then the cloud controller (1) pauses the NN inference task in the edge compute engine and cloud compute engine causing the video frames to wait in the queue, (2) modifies the tasks' parameters with the new partitioning point $x'$ (i.e., the end layer of edge task becomes x' and the start layer of cloud task becomes x' + 1), (3) resumes the execution with the new partitioning. The whole repartitioning procedure takes less than 1 second. 

{\bf Limitations:} One of the main advantages of our approach is leveraging pipelining which allows to utilize both edge and cloud servers. However, this is only applicable when the interarrival time between frames is less than the processing time of the entire NN for one frame. For example, if 1 frame comes to the system every 5 second and it is processed in 100 ms then there will be no pipelining because both edge and cloud resources will be idle waiting for the next frame. Our contribution is more pronounced when the interarrival time between frames is fast (e.g.,10 ms) which happens in two cases:(1) {\bf Real-time event analysis:} The edge device receives frames at real-time from multiple cameras; (2) {\bf Post-event analysis:} The semantically encoded video that is  being analyzed is pre-recorded and stored in the edge server. In this case, seeking I-frames is not bounded by the video capturing rate (e.g. 30 fps) and it goes beyond 2000 fps. In the cases when the interarrival time is large, we use the same algorithm with $n=1$ (i.e., no pipelining). 

It is worth mentioning that our goal is not to say that partitioning is always beneficial but to provide a systematic method to decide whether to partition or not. In Section~\ref{sec:eval}, we discuss the cases when our algorithm decides not to partition.
%benefecial is when the data from the NN intermediate layers is much larger transmission time of the intermediate 

%{\bf Chunk size (n):} We note that $n$ has an indirect impact on the partitioning point $x$. 

%{\bf Choosing chunk Size ($n$):} The size of $n$ depends on the number of events. If the number of events increases, then the number of I-frames increases and the interarrival times between I-frames will decrease which increases the need for pipelining. We empirically choose $n$ to be the biggest value that does not violate the pipelining assumption (i.e., ensures that the interarrival time is less than the NN processing time). In the extreme case, when the interarrival time between any two frames is greater than the NN processing time, we set $n$ to 1. The interarrival time can be inferred from the GOP size of the semantically encoded video. If the GOP size is 60 then we infer that one frame arrives to the NN inference engine every 2 seconds for live videos (30 fps) and one frame arrives every 30 ms for a pre-recorded videos (2000 fps). These interarrival times can be further reduced with increasing the number of camera feeds being analyzed. 


%We note that the value of $n$ has an impact on the interarrival time. The more the value of $n$, the more likely the interarrival will increase especially when there are infrequent events. Hence, we empirically choose $n$ to be the biggest value that does not violate the pipelining assumption (i.e., ensures that the interarrival time is less than the NN processing time). In the extreme case, when the interarrival time between any two frames is greater than the NN processing time, we set $n$ to 1. The interarrival time can be inferred from the GOP size of the semantically encoded video. If the GOP size is 60 then we infer that one frame arrives to the NN inference engine every 2 seconds for live videos (30 fps) and one frame arrives every 30 ms for a pre-recorded videos (2000 fps). These interarrival times can be further reduced with increasing the number of camera feeds being analyzed. 




%To address the limitation above, we choose the chunk size in a way that makes the interarrival time less than the processing time of the entire NN.  We note that the chunk size have an indirect impact on the partioning point $x$. If a chunk size  as long as the interarrival time is small.  as long as the number


%is the case when the data comes at real-time from multiple cameras or the video being analyzed is pre-recorded and stored in the edge server. 
%\begin{algorithm}
%\label{algo-nn-part}
%\caption{NN-Partition}

%\begin{algorithmic}[1]
%\State  \textbf{Input: } (1) Number of frames $n$ in chunk $k$, (2) profiling information for execution time of each layer in the edge and cloud, and the output data of each layer $P=\{L_i @ E, L_i @ C, D_{L_i}\}_{i=0}^{i=m}$, (3) Bandwidth from $E$ to $C$ ($B_{E,C}$) 
  
%\State \textbf{Output: } Partitioning layer $L_x$ 
%\State $L_x$ = $L_0$ 
%\State $t_{min}$ = MAX\_VALUE
%\For{i=0: m}
% \State $t_i$=\Call{CHUNK\_COMPLETION\_TIME}{$n,L_i,P,B_{E,C}$}
% \If{$t_i$ < $t_{min}$}
%\State $t_{min}$= $t_i$
%\State $L_x$ = $L_i$ 
%\EndIf
%\EndFor

%\Function{CHUNK\_COMPLETION\_TIME}{$n,L_i,P, B_{E,C}$}
% \State t =  $\big(n - 1\big)* max\big( \sum_{j=1}^{j=i} L_j@E, \frac{D_{L_{i}}}{B_{E,C}}, \sum_{p=i+1}^{p=m} L_p@C \big)$ +    $\sum_{j=1}^{j=i} L_j@E$ + $\frac{D_{L_{i}}}{B_{E,C}}$ + $\sum_{p=i+1}^{p=m} L_p@C)$
%\State \Return{t}
%\EndFunction
%\end{algorithmic}
%\end{algorithm}

%%Put the interarrival time in the picture, (Table of notation, pipelined execution section and figure, equations. 
%%State the pipelining assumption and justify that it works for multiple cameras or pre-recorded videos and that n and the GOP size somehow defines the interarrival time
%{\bf Chunk size (n):} We note that $n$ has an indirect impact on the partitioning point $x$. 


%To address the limitation above, we choose the chunk size in a way that makes the interarrival time less than the processing time of the entire NN.  We note that the chunk size have an indirect impact on the partioning point $x$. If a chunk size  as long as the interarrival time is small.  as long as the number 


%Maybe we can start with neural network model and data model

%Then go to the overview and pipelined execution

%Then among the algorithm steps start with profiling

